Forecast Collapse in Time-Series Foundation Models

When forecasting hourly returns for 1,000 US equities, we observe an unexpected phenomenon: predictions become nearly flat and show poor stock ranking, as measured by cross-sectional correlation. We call this forecast collapse. Surprisingly, the phenomenon largely disappears when forecasting trading volume under the same setting. We investigate forecast collapse across time-series foundation models (TSFMs), twelve deep-learning forecasting models, and 97 public benchmark configurations, and find that it is closely tied to target predictability. We identify two distinct reasons behind it: low predictability limits the amplitude of calibrated point forecasts, while per-series objectives leave cross-series structure unidentified. These findings reveal a calibration-ranking tradeoff: optimizing squared error leads to flat predictions, whereas directly optimizing cross-sectional correlation improves ranking but can inflate forecast amplitude by more than an order of magnitude. To address this tradeoff, we introduce CalibRank, a simple objective that balances calibration and ranking. On Finance1K, CalibRank nearly triples cross-sectional correlation while keeping amplitude close to the target, and improves correlation on all tested models. Our results reveal a blind spot in conventional time-series evaluation: per-series metrics can hide failures in cross-series structure needed by downstream decisions.

==> fonts/pdfmap.tex <==
\pdfmapline{+geist-regular--base Geist-Regular "AutoEnc_h4mqylmhebmidzuktqruwryivf ReEncodeFont" <[fonts/a_h4mqyl.enc <fonts/Geist-Regular.pfb}
\pdfmapline{+geist-semibold--base Geist-SemiBold "AutoEnc_h4mqylmhebmidzuktqruwryivf ReEncodeFont" <[fonts/a_h4mqyl.enc <fonts/Geist-SemiBold.pfb}
\pdfmapline{+geist-italic--base Geist-Italic "AutoEnc_h4mqylmhebmidzuktqruwryivf ReEncodeFont" <[fonts/a_h4mqyl.enc <fonts/Geist-Italic.pfb}

